UniGame: Turning a Unified Multimodal Model Into Its Own Adversary

Unified Multimodal Models (UMMs) have shown impressive performance in both understanding and generation with a single architecture. However, UMMs still exhibit a fundamental inconsistency: understanding favors compact embeddings, whereas generation favors reconstruction-rich representations. This structural trade-off produces misaligned decision boundaries, degraded cross-modal coherence, and heightened vulnerability under distributional and adversarial shifts. In this paper, we present UniGame, a self-adversarial post-training framework that directly targets the inconsistencies. By applying a lightweight perturber at the shared token interface, UniGame enables the generation branch to actively seek and challenge fragile understanding, turning the model itself into its own adversary. Experiments demonstrate that UniGame significantly improves the consistency (+4.6%). Moreover, it also achieves substantial improvements in understanding (+3.6%), generation (+0.02)on GenEval, out-of-distribution and adversarial robustness (+4.8% and +6.2% on NaturalBench and AdVQA). The framework is architecture-agnostic, introduces less than 1% additional parameters, and is complementary to existing post-training methods. These results position adversarial self-play as a general and effective principle for enhancing the coherence, stability, and unified competence of future multimodal foundation models. The official code is available at: https://github.com/AIFrontierLab/TorchUMM

==> figs/figtex/figure1.tex <==
\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{figs/consistency_intro.pdf}
  \caption{}
  \label{fig:figure1}
\end{figure}

==> figs/figtex/hard_loss.tex <==
\begin{figure}[H]
  \centering
  \includegraphics[width=\linewidth]{figs/hard_loss.png}
  \caption{Contribution of clean, adversarial, and mined-hard samples.}
  \label{fig:clean-adv-hard}
\end{figure}

==> script.tex <==

% [previous]
% Contributions.
% (1) \textbf{Novel formulation.} Formalize UMM co-training as a minimax game over a shared token interface. \textcolor{red}{[maybe we should highlight the impact?]}
% (2) \textbf{Plausible adversaries.} Introduce a lightweight Perturber that operates on visual tokens and—when decoded—produces semantically plausible adversarial images, enabling on-manifold hard examples.
% (3) \textbf{Stable co-training.} Propose perturbation budgets, regularizers, and hardness-aware mining schedules for stable, compute-efficient adversarial co-training of UMMs.




% \subsection{Discussion}
% \label{sec-method-discussion}

% \wjd{The difference between our work and GAN; show why it is nontrivial.}

% Empirically, we observe two key phenomena across UMMs: (i) structured token-space perturbations and adversarial embedding perturbations can expose real reasoning failures and improve robustness when used in training (cf. VILLA and token-perturbation work); (ii) unguided perturbations or purely embedding-level adversaries are often semantically implausible when decoded or destroy generation priors and degrade fidelity. 
% These findings imply that adversarial signals must be both semantically targeted and decodable into realistic visuals, so the understanding branch is exposed to believable hard cases rather than synthetic noise. 
% Injecting controllable perturbations at the shared visual-token interface and decoding them with the model’s own decoder yields on-manifold, visually plausible counterexamples; importantly, this makes the perturbation policy credit-assignable through a single computation graph, enabling a stable minimax game rather than cooperative fine-tuning.

% \textcolor{red}{[Mark: Which discussion version fits better here?]}




% \subsection{\textcolor{red}{Framework overview}}
% \label{sec:framework}

% We propose \textbf{\method}, a minimax self-play that treats the decoder as an active challenger.
% A lightweight Perturber parameterized by $\theta_C$ yields a bounded token perturbation $\boldsymbol{\delta}=\boldsymbol{\delta}(\mathbf{z};\theta_C)$ and produces perturbed tokens $\tilde{\mathbf{z}}=\mathbf{z}+\boldsymbol{\delta}$.
% The decoder decodes $\tilde{\mathbf{z}}$ to a visually plausible adversarial image $\tilde{\mathbf{x}}=G(\tilde{\mathbf{z}})$, which ensures attacks remain on the model's manifold.
% The language backbone (Defender) with parameters $\theta_D$ must answer queries conditioned on clean and perturbed tokens.
% The minimax objective we optimize is
% \begin{equation}
% \begin{aligned}
% \min_{\theta_D}\;\max_{\theta_C}\; \mathbb{E}_{(\mathbf{x},q,a)}\Big[ \; &
% \mathrm{CE}\big(p_D(a\mid \mathbf{z}+\boldsymbol{\delta}(\mathbf{z};\theta_C),q;\theta_D), a\big) \\
% & - \lambda \|\boldsymbol{\delta}(\mathbf{z};\theta_C)\|^2 \Big],
% \end{aligned}
% \label{eq:minmax_main}
% \end{equation}
% where the norm penalty bounds perturbation magnitude and prevents destruction of generative priors. Decoding plus an optional semantic-consistency regularizer (e.g., CLIP hinge) ensures adversarial examples are both decodable and semantically plausible.




% \subsection{Detailed design}
% \label{sec:design}
% The Gen-Challenger is a compact Perturber paired with the model's native decoder.
% The Perturber maps $\mathbf{z}$ to a token-wise output $\boldsymbol{\delta}$, clipped to $\|\boldsymbol{\delta}\|\le\varepsilon_{\max}$ to ensure boundedness. Its optimization balances attack strength, perturbation regularization and semantic plausibility:
% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{C}(\theta_C;\theta_D) =&\; \mathrm{CE}\big(f_D(\mathbf{z}+\boldsymbol{\delta},q;\theta_D),a\big) - \lambda\|\boldsymbol{\delta}\|^2 \\
% & + \gamma \big[\tau - s_{\mathrm{CLIP}}(G(\mathbf{z}+\boldsymbol{\delta}), q)\big]_+,
% \end{aligned}
% \label{eq:lossC}
% \end{equation}
% where $s_{\mathrm{CLIP}}(\cdot,\cdot)$ is a text–image similarity and $[\cdot]_+$ is the hinge.
% Each source yields $K$ decoded candidates; the challenger proposes those that maximize classification confusion while keeping CLIP similarity above a tolerance.

% The Und-Defender updates only language-side adapters (LoRA). Its loss mixes clean, current adversarial and mined hard samples:
% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{D}(\theta_D) =&\; \mathbb{E}_{\mathrm{clean}}\big[\mathrm{CE}(f_D(\mathbf{z},q;\theta_D),a)\big] \\
% & + \alpha\,\mathbb{E}_{\mathrm{adv}}\big[\mathrm{CE}(f_D(\mathbf{z}+\boldsymbol{\delta},q;\theta_D),a)\big] \\
% & + \beta\,\mathbb{E}_{(\mathbf{x},q,a)\in\mathcal{B}}\big[\mathrm{CE}(f_D(\mathbf{z},q;\theta_D),a)\big].
% \end{aligned}
% \label{eq:lossD}
% \end{equation}



% A mined hard-sample buffer $\mathcal{B}$ (capacity $B_{\max}$) stores tuples $(\mathbf{x},q,a,H)$ where each candidate's hardness is computed as
% \begin{equation}
% \begin{aligned}
% H_j &= \mathrm{CE}\big(f_D(G(\mathbf{z}+\boldsymbol{\delta}_j),q),a\big) \\
% &\quad + \lambda_{\mathrm{clip}}\,[\tau - s_{\mathrm{CLIP}}(G(\mathbf{z}+\boldsymbol{\delta}_j), q)]_+.
% \end{aligned}
% \label{eq:hardness}
% \end{equation}
% Per-source top candidates above a dynamic percentile (e.g., 80th) are pushed to $\mathcal{B}$; sampling from $\mathcal{B}$ uses a temperature $T_b$ to maintain diversity. Mining occurs every $m$ steps.

% Training alternates per mini-batch: (i) freeze $\theta_D$, update $\theta_C$ via AdamW to (approximately) maximize $\mathcal{L}_C$ and decode $K$ candidates for mining; (ii) freeze vision and decoder, update $\theta_D$ to minimize $\mathcal{L}_D$ on a mixed batch of clean, current adversarial and mined examples. This closed-loop alternation provides stable credit assignment: Defender gradients steer the attack policy via the maximization step, while decoded adversarial images ensure the attack stays on-manifold.


% \subsection{Discussion}

% Although our formulation involves a minimax objective and a decoder that renders visual samples, it differs fundamentally from conventional GANs. 
% GANs aim to \emph{learn} a data distribution via a generator–discriminator game \citep{Goodfellow2014}, while our Perturber–Defender setup operates \emph{within} a pre-trained Unified Multimodal Model (UMM) and exploits its shared visual–language token space. 
% Here, the decoder $G$ is not trained to generate new data but serves as a \emph{semantic renderer} that constrains perturbations to remain on-manifold and interpretable across modalities. 
% This decoder-constrained adversarial loop is nontrivial because (i) perturbations in UMM token space induce structured multimodal shifts, making simple embedding or pixel perturbations insufficient; (ii) the Perturber must maximize understanding loss while preserving cross-modal consistency; and (iii) the game remains fully differentiable through the UMM pipeline, enabling stable credit assignment without external discriminators.

% In essence, our framework performs \emph{task-driven adversarial mining} within the model’s own multimodal manifold, rather than distribution matching as in GANs. 
% This design reveals cross-modal reasoning weaknesses while maintaining semantic plausibility—an important distinction for UMM robustness and alignment research.


% \subsection{Preliminary}
% UMM is not a monolithic network, but rather a coupling of two pathways: understanding and generation~\citep{xx}.
% Although the two pathways share the image token embeddings used for generation, their optimization mechanisms are fundamentally heterogeneous: the understanding end optimizes for conditional language likelihood (e.g., describing what is in an image), while the generation end targets reconstruction or prior consistency (e.g., text-based image generation).
% \textit{Inconsistency} naturally emerges in such heterogeneous objectives between the understanding and generation capabilities: the priors and sampling stochasticity of the generation end may shift or interfere with discriminative decision boundaries, while gradients from the understanding end cannot constrain the priors and sampling strategies of the generation end.

% Conventional fine-tuning approaches normally consist of a single loss function, neither disentangling the mutual interference between the two pathways nor controllably rectifying such inconsistency.
% \wjd{summarize what existing work has done using references.}
% \wjd{Then, what is the key challenge they fail to resolve?}

% \subsection{UniGame}
% \wjd{Before jumping into our method, what is the motivation to propose this approach?}
% To address this, we propose \textit{\method}: leveraging Perturber as a controlled modulator to inject bounded, targeted perturbations, which are first materialized through generation-end decoding and subsequently fed back to the understanding end, thereby enabling the two pathways to mutually constrain each other within a closed loop and achieve reciprocal improvement through adversarial interplay.
% We are interested in dive into how understanding and generation moudules are interact with each other, We cast multimodal understanding–generation co-training as a min–max game between (i) a \emph{Gen-Challenger (C)} that injects perturbations into the image pathway to produce degraded yet semantically plausible visual evidence, and (ii) a \emph{Und-Defender (D)}, the UMM’s language backbone optimize to answer vision-grounded queries correctly. The Gen-Challenger combines a lightweight \textbf{Perturber} and UMM's \textbf{visual decoder}; it yields adversarial reconstructions, and when used inside the understanding path it yields adversarial features. The Und-Defender finetunes the attached lora layers of the LLM. We alternately update $D$ and $C$ once per batch.

% \paragraph{Uni-Challenger}
% Gen-Challenger comprises two components: UMM's Generation module, and a lightweight learnable Perturber. The Perturber operates on the shared projected visual tokens $z \in \mathbb{R}^{N \times H}$ (where $N$ is the number of tokens and $H$ the hidden dimension) that serve as the interface between vision encoding and both understanding and generation pathways. 
% The Gen-Challenger's objective is to maximize the understanding loss, formalized as:
% \begin{equation}
% \mathcal{L}_G = \mathrm{CE}(f_D(\tilde{z}, q), a) - \lambda \|\delta\|^2
% \label{eq:lg}
% \end{equation}
% Guided by this objective, the Gen-Challenger dynamically discovers failure modes of the understanding module and refines its perturbation strategy as the Defender becomes more robust.

% \paragraph{Uni-Defender}
% The Und-Defender is the Understanding model of the UMM. We freeze the vision tower and projector, and update only the LoRA modules. The Und-Defender minimizes loss on (i) \emph{clean} images and (ii) \emph{adversarial} images produced by the Gen-Challenger.

% \paragraph{Hard buffer.}
% We maintain a lightweight priority buffer of capacity $4096$ that stores tuples \{image tensor, question, GT answer, hardness score\}.
% Per batch we generate $K{=}3$ decoded candidates per instance, score each candidate $j$ with
% \[
% H_j \;=\; \mathrm{CE}\!\left(f(\tilde{x}_j,q),a\right)\;+\;\lambda_{\text{clip}}\,[\,\tau - s_{\text{CLIP}}(\tilde{x}_j,q)\,]_+,
% \]
% and keep per-source top-$k$ ($k{=}1$) above a dynamic threshold.
% Unless specified: $\tau{=}0.30$, $\lambda_{\text{clip}}{=}0.2$, buffer sampling temperature $T_b{=}2.0$, mined-batch size $8$, and mining stride $1$.
% This procedure balances \emph{answer difficulty} and \emph{text–image consistency}, continually refreshing challenging but semantically plausible examples.

% Candidate fanout $K$ (\verb|cand_K|, default 3),
% CLIP hinge $(\tau,\lambda_{\mathrm{clip}})$,
% per-source top-$k$,
% buffer sampling temperature $T_b$,
% and mining stride are configurable. We log paired clean/adv grids, mined panels, and an \emph{eps–step} curve.

% \paragraph{Min–max Game.}
% Our key idea is to test if self training can be promising for UMMs, 

% For each mini-batch:
% \begin{enumerate}
%     \item \textbf{Step 1.} Enable Gen-Challenger, freeze LLM; maximize $\mathcal{L}_G$ (Eq.~\ref{eq:lg}) by AdamW.
%     \textbf{(2)Hard Sample Mining:} Every $m$ steps, generate $K{=}3$ candidates per sample. 
%     Score by $H_j{=}\mathrm{CE} + \lambda_{\text{clip}} \max(0, \tau - s_{\text{CLIP}})$. 
%     Keep top-1 per source above 80th percentile of $H$; push to buffer (cap. 4096).
%     \item \textbf{Step 2.} Enable only the LLM’s last layers/adapters; minimize $\mathcal{L}_D$ (Eq.~\ref{eq:ld}) via (i) decoded adversarial images, (ii) clean images, and (iii) mined hard images. Use small LR ($10^{-5}$–$2{\times}10^{-5}$).
% \end{enumerate}

% \subsection{Implementation Details}
% \paragraph{Backbone.}
% Instantiated with Janus-Pro-7B as the UMM; vision and projector are frozen. The LM is LoRA-augmented; only Lora and Perturber can receive gradients.

% \paragraph{Optimizers \& hyperparameters.}$\varepsilon_{\max}{=}0.02$, \verb|img_gen_size| $=384$, \verb|patch_size| $=8$, \verb|cfg_weight| $=5.0$.


% Crucially, we empirically observe two phenomena across UMMs: (i) structured token-space perturbations and adversarial embedding perturbations often expose real reasoning failures (c.f. VILLA, token-perturbation work in VLM), improving downstream robustness when used in training; (ii) however, unguided perturbations (random/noise) or purely embedding-level adversaries tend to either (a) be semantically implausible when decoded, or (b) destroy generation priors and degrade fidelity. These observations suggest a design need: adversarial signals should be both semantically targeted and decoded into plausible visuals so that the understanding branch sees realistic hard cases rather than synthetic embedding noise. 

% \begin{figure}[htbp] 
%   \centering
%   \includegraphics[width=\linewidth]{figs/intro2.png}
%   \caption{UniGa enables self-improvement in robustness.}
%   \label{fig:intro2}
% \end{figure}

% If we inject controllable perturbations directly at the shared visual-token interface and decode them with the model’s own generate module, we obtain on-manifold, visually plausible counterexamples that are maximally informative for its own. Crucially, the loss becomes credit assignable to the perturbation policy along a single, consistent computation graph—enabling a stable min–max game rather than cooperative fine-tuning.


% Motivated by this, we propose UniGa: a selfplay loop that treats generation as an active adversary for UMMs. A lightweight perturber crafts bounded perturbations in the shared token/embedding interface; perturbations are (i) injected into the understanding pathway as adversarial conditioning and (ii) decoded by the model’s native generation module into visually plausible adversarial images. The understanding branch acts as the Und-Defender; its gradients steer perturber toward the most informative, plausible failure cases.






% Despite these advances, a fundamental tension remains. Academic work on post-training remains limited and has not crystallized into a unified paradigm. Understanding objectives favor compact, discriminative embeddings optimized for tasks, while generation objectives favor reconstruction-rich representations that preserve fine visual detail; optimizing both together produces competing gradients and ambiguous shared interfaces, which can cause brittle cross-modal reasoning and hidden failure modes. For example, the same UMM that faithfully reconstructs the scene in pixel space nonetheless answers a simple counting/attribute query incorrectly under occlusion. This gap shows that a unified architecture does not guarantee unified behavior; it calls for a post-training mechanism that explicitly couples the generative and discriminative pathways.



% These competing objectives produce conflicting gradients and ambiguous shared interfaces, causing brittle cross-modal reasoning and hidden failures. 


% Recent industrial systems (e.g., Janus-pro, BLIP-3-o, Chameleon) typically follow a staged recipe—web-scale pretraining, adapter alignment, and supervised finetuning (often with preference/RL) coupled to a decoder. Most of the post-train method can be category into:
% (i) reconstruction/alignment methods make the generation follow the understanding branch (unified reconstruction or semantic reconstruction),
% (ii) unified RL/GRPO optimizes global rewards with external evaluators.
% (iii) generation-side RL/CoT strengthens planning and fidelity.
% All three mitigate mismatch, but none turns generation into an adversary that actively exposes decision critical failures for the understanding branch to learn from. This cooperative framing leaves a missing piece and motivates our key idea.

% Prior solutions follow complementary directions. One stream redesigns tokenizer/encoding (e.g., TokenFlow, Chameleon, Janus) to provide different granularities for understanding and generation, mitigating representational conflict at the input stage. 

% Another stream uses alignment or reconstruction objectives (e.g., RecA) or stronger generation planning/reasoning (e.g., T2I-R1) to reduce modality mismatch or improve generation quality. 
% Both classes help, but neither fully treats generation as an active mechanism to reveal semantically plausible failure cases that the understanding branch must learn to resist.

==> tables/tab-perturb-budget.tex <==
\begin{table}[t]
\centering
\caption{Ablation on perturbation budget $\varepsilon_{\mathrm{max}}$. We fix $\tau{=}0.30$, $\lambda_{\mathrm{clip}}{=}0.2$, $K{=}3$, buffer size${=}4096$ and report VQAv2 accuracy (\%) after 10k training steps.}
\label{tab:ablation-eps}
\small
\begin{tabular}{@{}lc@{}}
\toprule
$\varepsilon_{\mathrm{max}}$ & Accuracy \\
\midrule
0.000 (no pert.) & 78.2 \\
0.005 & 80.5 \\
0.010 & 82.1 \\
\rowcolor{tblhilite}
\textbf{0.020} & \textbf{83.4} \\
0.030 & 83.2 \\
0.050 & 82.3 \\
0.100 & 79.8 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table-clip-ablation.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on CLIP constraint configurations. We fix $\varepsilon_{\max}=0.02$, $K=3$, and buffer size$=50$. We report VQAv2 accuracy (\%) for different combinations of $\lambda_{\text{clip}}$ (CLIP penalty weight) and $\tau$ (CLIP similarity threshold).}
\label{tab:ablation-clip}
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{\textbf{$\lambda_{\text{clip}}$}} & \multicolumn{6}{c}{\textbf{$\tau$ (CLIP similarity threshold)}} \\
\cmidrule(lr){2-7}
& \textbf{0.0} & \textbf{0.20} & \textbf{0.25} & \textbf{0.30} & \textbf{0.35} & \textbf{0.40} \\
\midrule
\textbf{0.0} & -- & -- & -- & -- & -- & -- \\
\textbf{0.1} & -- & -- & -- & -- & -- & -- \\
\textbf{0.2} & -- & -- & -- & -- & -- & -- \\
\textbf{0.5} & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table}
